How Well Do LLMs Identify Cultural Unity in Diversity?

Much work on the cultural awareness of large language models (LLMs) focuses on the models' sensitivity to geo-cultural diversity. However, in addition to cross-cultural differences, there also exists common ground across cultures. For instance, a bridal veil in the United States plays a similar cultural-relevant role as a honggaitou in China. In this study, we introduce a benchmark dataset CUNIT for evaluating decoder-only LLMs in understanding the cultural unity of concepts. Specifically, CUNIT consists of 1,425 evaluation examples building upon 285 traditional cultural-specific concepts across 10 countries. Based on a systematic manual annotation of cultural-relevant features per concept, we calculate the cultural association between any pair of cross-cultural concepts. Built upon this dataset, we design a contrastive matching task to evaluate the LLMs' capability to identify highly associated cross-cultural concept pairs. We evaluate 3 strong LLMs, using 3 popular prompting strategies, under the settings of either giving all extracted concept features or no features at all on CUNIT Interestingly, we find that cultural associations across countries regarding clothing concepts largely differ from food. Our analysis shows that LLMs are still limited to capturing cross-cultural associations between concepts compared to humans. Moreover, geo-cultural proximity shows a weak influence on model performance in capturing cross-cultural associations.

==> figs/06_results/geoculture/geoculture.tex <==
\begin{figure}[h]

\begin{center}
 \centering
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{figs/06_results/geoculture/geo_culture_with_features.png}
    \end{minipage}
    %\qquad
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{figs/06_results/geoculture/geo_culture_without_features.png}
    \end{minipage}
\end{center}
\caption{\textbf{Performance of the model across countries.} The worse performance indicates that the selected cultural concepts between the two countries are more difficult to distinguish.}
\label{fig:geoculture}
\end{figure}

% 需要标注是否是GPT的值，单独计算with w/o features

% right / all

% 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/backup.tex <==
%Our work select \textbf{Cultural Concept Alignment} as the evaluation task on the benchmark dataset. Specifically, given cultural concept $c_1$ from country A and $c_2, c_3$ from country B, we generated $Sim(c_1, c_2), Sim(c_1, c_3)$ as the real labels, and require large language models to measure the size relationship between $Sim(c_1, c_2)$ and $Sim(c_1, c_3)$.

%We first provide a definition of a \emph{cultural association} by referring to prior work in intercultural communication \citep{icctheory, doi:10.1177/0193945905284712}: Given two concepts $c_i$ and $c_j$, a \textbf{cultural association} is defined as the similarity of culturally relevant communicative effect (e.g., cultural significance) conveyed by these two concepts. Extending from this definition, we specify the \textbf{cross-cultural association} as the cultural association between two concepts that originate from different cultures. 

%The construction of \textbf{CulComp} benchmark dataset can be defined as an alignment task among cross-cultural concepts, formally speaking:
% \vspace{-0.5em}
% \begin{itemize}[leftmargin=10pt] \itemsep-0.2em
%     \item \textit{Given:} a set of cultural-specific concepts $\mathcal{C} = \{c_1, c_2, \dots, c_n\}$ and their descriptions $\mathcal{D_C} = \{d_{c_1}, d_{c_2}, \dots, d_{c_n}\}$.
%     \item \textit{Goal:} calculate the cross-cultural association $\mathcal{S} = \{Sim(c_i, c_j)\}$ between any pair of cross-cultural concepts based on their descriptions.
% \end{itemize}
% \vspace{-0.5em}

% The details of our data curation process are described below.

%We first provide a definition of a \emph{cultural association} by referring to prior work in intercultural communication \citep{icctheory, doi:10.1177/0193945905284712}: Given two concepts $c_i$ and $c_j$, a \textbf{cultural association} is defined as the similarity of culturally relevant communicative effect (e.g., cultural significance) conveyed by these two concepts. Extending from this definition, we specify the \textbf{cross-cultural association} as the cultural association between two concepts that originate from different cultures. 

%Intuitively, our concentration on concept-level cultural unity emphasizes the cultural-centered pragmatic similarity. Following this intuition, 




%In order to obtain different cultural concept triplets, our work calculates the similarity between all collected cultural concepts, and combines cultural concept pairs with the same concept into cultural concept triplets (including cultural concept $c_1$ from country A; $c_2, c_3$ from country B), in order to study the regional difference ability of the large language model, we ensured that the countries where $c_2$ and $c_3$ are located are the same during the construction process.
%We divide all cultural concept triples into three granularities: large, middle and small (shown in the Table~\ref{tab:three_granularity}) according to the difference between $ Sim(c_1, c_2)$ and $Sim(c_1, c_3)$, and in order to improve the visibility of real labels Reliability, we artificially require that among $Sim(c_1, c_2)$ and $Sim(c_1, c_3)$, one is greater than 0.5 and the other is less than 0.5, so as to avoid that the two pairs of cultural concepts are both very similar or not similar.


%\paragraph {Prompting}



%By setting different similarity thresholds, cultural concept pairs with similar features were combined into triples. These triples take the form of $concept_1$ from $country_A$ and $concept_2$, $concept_3$ from $country_B$. These triples were then used to construct the test set for evaluating the performance of large language models, as shown in the right half of Figure~\ref{fig:pipeline}.

%\textbf{Geo-culture selection.} In various geographical cultures, a statistical ranking was conducted based on the number of entries related to clothing concepts in the countries listed on Wikipedia. The countries with high entries for clothing were selected from different continents (shown in Table~\ref{tab:clothing_concept}). Additionally, considering the substantial number of entries for India, China, and Japan among Asian countries, five Asian countries centered around India, China, and Japan were chosen. For other continents, the countries with high number of entries were selected, and the cultural-specific concepts of these countries were used as the research subjects.

%\ljl{The processes of Geo-culture and concept selection are written in Chinese in the comments section:
% 由于模板的原因，不能直接写中文，因此用注释的形式
% Geo-culture selection
% 1. 从wikipedia中不同国家的category获取不同的文化概念，选取了不同国家的category，例如Chinese food, Chinese clothing, ..., 分别统计了不同国家的cultural concept的数目总和，从不同的大洲中分别选取了concept较为丰富的国家（即Geo-cultural）
% 2. 为了调研地域临近是否会对大语言模型产生更大的影响，在亚洲范围内额外选取了日本，韩国，泰国这些国家，便于进一步探究地域临近对模型效果的影响
% （以下属于是concepts selection的部分，本质上不属于Geo-culture selection）
% 3. 从所选取的geo-culture当中的category下获取不同的concepts，并对全量的food和clothing concept进行了标注
% 4. 首先使用chatgpt帮助我们筛选出所有wikipedia的文本中的描述性语言
% 5. 人工标注者结合wikipedia中的原文和gpt筛选后的描述性语言，截取出文本中的描述性词语，此时的描述性词语仍然是不规则的，可能包含短语，原文中的符号，将描述性词语分为user，occasion，significance三个大类
% 6. 筛选去除特征较少的concept，具体来说，将三个大类中至少缺少两个大类的concept删除了
% 7. 数据清洗（也包括了正则化的步骤）：把已有的描述性短语进行清洗，去除乱码和符号，同时把类似的描述性词语归一化为相同的表述（例如，joy, happy, cheerful都归一化为happiness），用相同的表述来表示相似的描述性短语
% }

%\textbf{Formal definition of cultural-specific concept.} Culture is a broad concept, and there should be different definitions of cultural-specific concept for different research questions. In our work, we define the cultural-specific concept as "tangible products and items shared and inherited within specific geographical areas and communities." More specifically, our cultural-specific concepts are derived from the pages under the Wikipedia category "Culture by country". We have selected clothing concepts from different countries as the cultural-specific concepts in our research. Taking clothing as the example, the features of clothing vary in different regions when considering aspects such as wearer, attendance occasion, and symbolic meaning.

%\textbf{Formal definition of cross-cultural correlations between concepts.} In our research, we prioritize the evaluation of language models based on their ability to comprehend the distinctive features of cultural-specific concepts and measure the relationships between these concepts. To achieve this goal, we focus on investigating the "similarity relationships" between cultural concepts. For cultural-specific concepts $A$ and $B$, we select features related to a particular aspect $f$(using clothing as an example: wearer, attendance occasion, and symbolic meaning, etc.). We quantify the similarity $S$ between cultural-specific concepts $A$ and $B$ by computing the Jaccard similarity coefficient of aspect $f$.

% \begin{equation}
% S(A,B)=\dfrac{A_f\cap{B_f}}{A_f\cup{B_f}}
% \label{similarity}
% \end{equation}

% where $A_f$ and $B_f$ respectively represent the feature words of $A$ and $B$ in aspect of $f$.

% \textbf{Formal definition of cross-cultural association between concepts.}

%\subsection{Task Definition}
% \label{subsec:task_definition}

% % Cross-cultural association graph generation

% In this research, we employ the similarity between cultural-specific concepts as an evaluation task named ``Cross-cultural Concepts Alignment'' for large language models. Assessing the similarity between cultural concepts involves not only understanding the features of these concepts but also measuring the differences between the features of different cultural-specific concepts. This evaluation can test whether the knowledge learned by large language models during the pre-training stage contains cultural concepts, and whether the language model can accurately compare different feature words.

% \input{tables/gen_to_con_questions}

% To avoid potential issues with the illusion problem when directly generating answers and to facilitate annotators in annotating the answers of large language models, we convert the task into a comparison of similarity between different pairs of cultural concepts (shown in Table \ref{tab:gen_to_con_questions}). The input to the task consists of $concept_1$ from $country_A$ and $concept_2$, $concept_3$ from $country_B$. The output is a ranking of the similarity between $(concept_1, concept_2)$ and $(concept_1, concept_3)$. We use this task to evaluate whether large language models can correctly compare differences between different cultural concepts. Compared with generative questions, contrastive questions ensures a focused assessment of the model's ability to discern and compare cultural features, mitigating potential challenges associated with hallucinatory responses during direct answer generation. Generative questions are also helpful for labeling answers.



%\subsection{Dataset Collection}


%In this section, we introduce in detail the pipeline(shown in Figure \ref{fig:pipeline}) that constructs the test set used for evaluation: (1) Geo-culture selection, (2) Cultural-relevant feature extraction, (3) Pairwise cross-cultural correlations calculation, and (4) Generate prompts through different prompt strategies.

%\textbf{Geo-culture selection.} In various geographical cultures, a statistical ranking was conducted based on the number of entries related to clothing concepts in the countries listed on Wikipedia. The countries with high entries for clothing were selected from different continents (shown in Table~\ref{tab:clothing_concept}). Additionally, considering the substantial number of entries for India, China, and Japan among Asian countries, five Asian countries centered around India, China, and Japan were chosen. For other continents, the countries with high number of entries were selected, and the cultural-specific concepts of these countries were used as the research subjects.

% [NEED COUNTRY TABLE]

%\textbf{Cultural-relevant feature extraction.} For each cultural-specific concept, relevant descriptions from the Wikipedia pages were extracted, and features were categorized based on different aspects. For clothing concepts, features were extracted based on the three dimensions of wearer, attendance occasion, and symbolic meaning. After obtaining features from multiple dimensions of cultural-specific concepts, a unified classification structure was created through manual labeling.



%\textbf{Generate prompts through different prompt strategies.} According to the similarity difference between $(concept_1, concept_2)$ and $(concept_1, concept_3)$ in each cultural-specific concepts triples, we divide the generated triples according to different granularity (shown in \cref{sec:probing_design}). For LLMs, triples of different difficulties are obtained. Then we generate prompts through different prompt strategies.

%During testing with different models, we conducted two repeated experiments on candidate options with two different orders (forward and reverse), and observed a certain difference in accuracy between the two orderings across multiple experiments. Our work conducted relevant tests using consistency as a comparable metric. Figure~\ref{fig:consistency} shows the consistency of different models under different prompting strategies. It can be noted that gpt-3.5-turbo-0613 significantly outperforms the llama series models in consistency. This reflects that gpt-3.5-turbo-0613's analysis is less susceptible to the influence of order, resulting in higher quality responses.


%Further looking into two LLaMA variants, similar to prior work [XXX], we find that the 13B variant tends to show a higher comparison accuracy compared with the 7B variant. 



% \input{tables/06_results/final_results}

% \input{tables/06_results/final_results_wo_features}

% \input{tables/06_results/final_results_wo_concept_names}

% \input{tables/06_results/final_results_total}


%Our work focused on whether to give external features and conducted two sets of experiments (shown in Table \ref{tab:final_results}). The prompt words in experiments of upper half of the table incorporate external features related to cultural concepts, examining whether the model can better compare the relationships between different cultural-specific concepts when external knowledge is provided. Meanwhile, the prompt words in experiments of lower half of the table do not include features related to cultural concepts, examining the model's pre-training knowledge.

%Overall, gpt-3.5-turbo-0613 maintains the highest accuracy in almost all categories among the tested models. Additionally, llama-2-13b-chat outperforms llama-2-7b-chat in accuracy across multiple categories.

%\subsection{Prompting Strategy Comparison}



%\subsection{Intrinsic Model Biases}
% \begin{itemize}
%     %\item Effect of increasing prompting examples
%     \item Effect of prompting strategies
%     \item Effect of different models
% \end{itemize}

%We observed the impact of long-tail degree on LLMs' responses. In Figure\ref{fig:longtail_acc_gpt}, we compiled the maximum long-tail degree (denoted as $d_{max}$) among different cultural concept triplets. We presented the performance of the GPT model when $d_{max}$ is positioned in the top 33\% and bottom 33\%. The results indicate that the group with higher $d_{max}$ consistently exhibits higher accuracy on the GPT model compared to the group with lower $d_{max}$. In the computation of average accuracy under various degrees of long-tail degree, we excluded triplets affected by order bias and format errors. Detailed information regarding error analysis is presented in the Figure~\ref{fig:error_analysis} in the Appendix~\ref{sec:appendixD}.

%To further mitigate the influence of long-tail degree, we propose a potential method to eliminate its impact. Building upon experiments with features, we removed concept names (as shown in the Table~\ref{tab:final_results_wo_cocept_names}). Through this method, we alleviated the differences in long-tail degree caused by concept names, enabling the model to answer questions solely based on provided features. However, in this experiment, we observed that the llama series models are significantly affected by order bias and struggled with reasoning. The error analysis of LLaMA series model in the experiment without names in Figure~\ref{fig:error_analysis} can well demonstrate this point.




% \input{figs/06_results/geoculture/geoculture}

% We also conducted an analysis of the experimental results based on geographic regions. We selected the gpt-3.5-turbo-0613 model, which performed relatively well, to examine its performance under different prompting strategies. It can be noticed that the proportion of correct answers regarding relationships between cultural concepts varies across different countries. Particularly, lower accuracy rates between certain pairs of countries suggest that the cultural concepts selected from these countries are closer and less easily distinguishable from each other.

%In this section, we conducted a comprehensive analysis of the dataset from four perspectives: (1) quality analysis, (2) cultural variation, (3) long-tail degree of cultural-specific concepts, and (4) cross-cultural correlations distribution.

% \subsection{Quality Analysis}
% human evaluation





%\input{tables/03_dataset/all_concept_triples}

% Due to the necessity of manually extracting features from Wikipedia pages in our dataset, and a unified classification structure was manually created within the existing features of cultural concepts in constructing the dataset. As a result, there may be potential subjective factors affecting the quality of the dataset during the annotating process, subsequently influencing the quality of the test set used for evaluating language models. To ensure the reliability of the experiments, we employed manual assessment to guarantee the quality of the dataset.

% Due to the necessity of manually extracting features from Wikipedia pages in our dataset, and a unified classification structure was manually created within the existing features of cultural concepts in constructing the dataset. To ensure the reliability of the experiments, we employed manual assessment to guarantee the quality of the dataset. 

% Specifically, we selected 100 clothing concepts with the most features from five neighboring Asian countries: India, China, Japan, South Korea, and Thailand. A new annotator re-annotated these 100 cultural concepts. We calculated the Cohen's kappa coefficient between the original dataset and the data annotated by the new annotator is 0.9391. The results indicated a good consistency between the new annotations and the original annotations, demonstrating the comprehensiveness of the features extracted in our dataset. And we also show the performance of human annotators on the benchmark(shown in Table~\ref{tab:final_results}, \ref{tab:final_results_wo_features}).

% \input{tables/04_dataanalysis/cohen_kappa}

% In addition, for the test sets generated based on different granularity, we also conducted human evaluation (shown in the Table \ref{tab:human_evaluation}). Different annotators directly annotate the test set to evaluate its quality. Two annotators were employed, each using different additional information for annotation: (1) annotation solely based on information from Wikipedia, and (2) annotation exclusively using the feature table we extracted. In this manner, we simulated two scenarios: (1) LLMs answering questions without additional information, relying solely on raw data from the pre-training stage, and (2) LLMs answering questions when provided with some additional information. The purpose of the human evaluation is to ensure the authenticity and reliability of the labels in our test data. Overall, the kappa coefficients of the two annotators and the original test set perform well, proving that the triples we generated are reliable.

% \input{tables/04_dataanalysis/human_evaluation}

%Our benchmark includes 1425 QA testing pairs, covering 285 traditional cultural concepts from 10 countries spanning 5 continents(shown in Table~\ref{tab:clothing_concept}). And our work counts the distribution of countries where different concept triplets are located(shown in Table~\ref{tab:concept_triples}).




% \subsection{Long-tail Degree of Cultural Concept}
% e.g., google search engine \#webpages; google Ngram

%Our work conduct a long-tail degree analysis on the cultural concepts collected in \dataset using the Google search engine. Specifically, 1. We concatenate the cultural concept names with the corresponding countries to form queries as $Query=(concept\ name, country)$, 2. We directly query these queries using the Google search engine, 3. We count the number of returned web pages as the long-tail degree measure for each cultural concept.

% Chinese
% 我们的工作借助google search engine，在CUNIT收集到的文化概念上进行了长尾度分析。具体来说，1. 我们将文化概念名和国家拼接在一起，组成Query=(concept name, country)，2. 使用google search engine直接查询Query，3. 统计返回到的网页数目作为每个文化概念的长尾度

% In the process of evaluation, we observed that when LLMs trying to directly output cultural-specific concepts with certain rules, the models tend to favor culturally rich concepts. For instance, when using different types of clothing concepts from various countries (such as the Indian Sari) as input and requesting the model to generate a culturally equivalent Chinese outfit, the model often produces the response of "Cheongsam" or "Qipao" (a traditional Chinese dress). Therefore, we conducted a long-tail analysis (shown in Figure~\ref{fig:longtail_degree} and Figure~\ref{fig:longtail_acc_total} in Appendix~\ref{sec:appendixA}) on the cultural-specific concepts in the test set. Specifically, we formed queries $Q$ by combining cultural-specific concepts with the countries they are associated with. And we calculated the relationship between long-tail degree and the accuracy of different models. We utilized a programmable search engine within the Google engine to calculate the number of pages corresponding to each query $Q=(concept, country)$.

% Analyzing the long-tail distribution of existing cultural-specific concepts helps us identify potential edge cases, allowing for a more robust evaluation of the performance of large language models in specific scenarios. Additionally, this approach aids in uncovering peculiarities in the data distribution of cultural-specific concepts.

% [TABLE of long-tail analysis]

% \subsection{Cross-cultural association distribution}
% Cultural diversities and shared tendencies over countries \\
% Geo-cultural representativeness \\
% Geo-cultural proximity \\


==> tables/03_dataset/all_concept_triples.tex <==
\begin{table}[t]

\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccc} 
\toprule
\bf Category & \bf Granularity & \bf China & \bf India & \bf Japan & \bf Korea & \bf Thailand & \bf Australia & \bf America & \bf Mexico & \bf Italy & \bf Nigeria \\ 
\midrule
\multirow{3}{*}{Clothing} & Large  & 24 &  8 & 59  & 96 & 26 & 12 &   0 & 105 & 105 & 27  \\
                          & Middle & 53 & 25 & 81  & 78 & 19 & 34 &  27 &  14 &  95 & 16  \\
                          & Small  & 57 & 66 & 121 & 86 &  4 & 57 &   9 &   6 &  66 & 24  \\
\midrule
\multirow{3}{*}{Food}     & Large  & 22 & 82 & 16  & 0  &  6 &  0 &  52 &   0 & 134 &  0  \\
                          & Middle & 38 & 68 & 14  & 8  &  0 & 17 & 158 &   6 & 148 &  3  \\
                          & Small  & 73 & 83 & 44  & 18 &  0 & 37 & 176 &  14 & 229 &  4  \\
\bottomrule
\end{tabular}}
    
\end{center}

\caption{\textbf{The number of cultural-specific concept triplets of different countries.} Our work calculates the country distribution of cultural-specific concept triplets in different similarity groups. Specifically, each cultural concept triplet includes a query country(including query concept $c_1$) and a target country(including candidate concepts $c_2$ and $c_3$). We count the frequency of occurrence of each country(as query country or target country) in all concept triplets of \dataset.}
\label{tab:concept_triples}
\end{table}

==> tables/04_dataanalysis/cohen_kappa.tex <==
\begin{table}[t]

\begin{center}

\begin{tabular}{cc} 
\toprule
\bf Kappa coefficient & \bf Kappa coefficient(w/o consistent concepts)  \\ 
\midrule
0.9391                  & 0.8444                                                                                      \\
\bottomrule
\end{tabular}
\end{center}

\caption{\textbf{Cohen kappa consistent in sampling testing.} Cohen Kappa coefficient is the average of all cultural-specific concepts, and Cohen Kappa coefficient(w/o consistent concepts) is the average after removing completely similar cultural-specific concepts.}
\label{tab:cohen_kappa}
\end{table}

==> tables/04_dataanalysis/human_evaluation.tex <==

\begin{table}[t]

\begin{center}
    
\begin{tabular}{cccc} 
\toprule
\bf Granularity & \bf Testing Pairs & \bf Wikipedia annotator & \bf Feature annotator  \\ 
\midrule
Clothing-Large            &       231       &       93.51\%      &            100.00\%      \\ 
%\hline
Clothing-Middle            &       221       &      88.69\%      &            95.93\%       \\ 
%\hline
Clothing-Small           &       248       &        66.53\%         &         79.44\%         \\
Clothing-All            &       700       &        82.43\%         &         91.43\%         \\
Food-Large            &       156       &       91.67\%      &            94.87\%      \\ 
%\hline
Food-Middle            &       230       &      64.35\%      &            81.74\%       \\ 
%\hline
Food-Small           &       339       &        67.55\%         &         76.70\%         \\
Food-All            &       725       &        71.72\%         &         82.21\%         \\
\bottomrule
\end{tabular}

\end{center}

\caption{\textbf{The results of human evaluation.} Similar threshold is the cultural-specific concept of different degrees of similarity we selected. Wikipedia annotator and Feature table annotator means the accuracy of two different annotators using different information. It can be observed that as the similarity between cultural-specific concepts gradually becomes smaller, the accuracy of human annotators is also declining, especially the annotators who use Wikipedia as the data source. It shows that the concepts are harder to distinguish at \textit{Small} granularity.}
\label{tab:human_evaluation}
\end{table}

==> tables/05_experiment/LLM_models.tex <==
\begin{table}

\begin{center}

\begin{tabular}{ccc} 
\toprule
\bf Model Family & \bf Model   & \bf Parameter  \\ 
\midrule
GPT & gpt-3.5-turbo-0613           &         N/A                    \\
Llama & llama-2-7b-chat          &             7B                \\
Llama & llama-2-13b-chat           &           13B                   \\
\bottomrule
\end{tabular}

\end{center}

\caption{\textbf{Large Language Models.} Different series of large models are selected for evaluating in our work.}
\label{tab:LLM_list}
\end{table}

==> tables/06_results/final_results.tex <==
\begin{table}

\begin{center}

\resizebox{\textwidth}{!}{
\begin{tabular}{clccccccccc} 

\toprule
\multirow{2}{*}{\bf Category}          & \multirow{2}{*}{\bf Model} & \multicolumn{3}{c}{\bf Directly} & \multicolumn{3}{c}{\bf Oneshot} & \multicolumn{3}{c}{\bf CoT}  \\
\cmidrule{3-11}
                                   &                        & \bf Large     & \bf Middle     & \bf Small                      & \bf Large     & \bf Middle     & \bf Small                     & \bf Large     & \bf Middle     & \bf Small                  \\ 
\midrule
\multirow{4}{*}{\textit{Clothing}} & human                  & $100.0_{\pm 0.00}$ & $95.93_{\pm 0.00}$ & $79.44_{\pm 0.00}$                  & \textemdash & \textemdash & \textemdash                 & \textemdash & \textemdash & \textemdash              \\
                                    & gpt-3.5                & $\textbf{50.14}_{\pm 0.40}$ & $\textbf{54.82}_{\pm 0.00}$ & $\textbf{46.03}_{\pm 0.57}$                  & $\textbf{52.31}_{\pm 0.53}$ & $\textbf{55.88}_{\pm 0.56}$ & $44.69_{\pm 0.50}$                 & $\underline{\textbf{58.37}}_{\pm 0.89}$ & $\underline{\textbf{60.78}}_{\pm 1.30}$ & $\underline{\textbf{52.41}}_{\pm 0.50}$              \\                                  
                                   & llama-13b              & $41.99_{\pm 0.00}$ & $38.01_{\pm 0.00}$ & $40.32_{\pm 0.00}$                  & $49.13_{\pm 0.00}$ & $\underline{49.32}_{\pm 0.00}$ & $\underline{\textbf{50.00}}_{\pm 0.00}$                 & $\underline{49.78}_{\pm 0.00}$ & $48.87_{\pm 0.00}$ & $49.60_{\pm 0.00}$              \\
                                    & llama-7b               & $36.80_{\pm 0.00}$ & $30.32_{\pm 0.00}$ & $37.50_{\pm 0.00}$                  & $38.10_{\pm 0.00}$ & $39.37_{\pm 0.00}$ & $41.33_{\pm 0.00}$                 & $\underline{47.62}_{\pm 0.00}$ & $\underline{50.00}_{\pm 0.00}$ & $\underline{48.39}_{\pm 0.00}$              \\
                                    
\midrule
\multirow{4}{*}{\textit{Food}}     & human                  & $94.87_{\pm 0.00}$ & $81.74_{\pm 0.00}$ & $76.70_{\pm 0.00}$                  & \textemdash & \textemdash & \textemdash                 & \textemdash & \textemdash & \textemdash              \\ 
                                    & gpt-3.5                & $\textbf{65.81}_{\pm 0.30}$ & $\textbf{52.32}_{\pm 0.41}$ & $\underline{43.66}_{\pm 0.00}$                  & $\textbf{65.92}_{\pm 0.60}$ & $\underline{\textbf{57.10}}_{\pm 0.71}$ & $37.81_{\pm 0.37}$                 & $\underline{\textbf{67.20}}_{\pm 0.30}$ & $\textbf{51.81}_{\pm 1.34}$ & $36.68_{\pm 0.77}$              \\
                                   & llama-13b              & $46.47_{\pm 0.00}$ & $\underline{48.26}_{\pm 0.00}$ & $\underline{\textbf{46.90}}_{\pm 0.00}$                  & $\underline{49.68}_{\pm 0.00}$ & $47.17_{\pm 0.00}$ & $\textbf{46.46}_{\pm 0.00}$                 & $45.51_{\pm 0.00}$ & $46.52_{\pm 0.00}$ & $44.40_{\pm 0.00}$              \\
                                   & llama-7b               & $40.71_{\pm 0.00}$ & $38.48_{\pm 0.00}$ & $42.63_{\pm 0.00}$                  & $50.32_{\pm 0.00}$ & $38.26_{\pm 0.00}$ & $41.74_{\pm 0.00}$                 & $\underline{52.24}_{\pm 0.00}$ & $\underline{50.00}_{\pm 0.00}$ & $\underline{\textbf{47.05}}_{\pm 0.00}$              \\
\bottomrule
% \hline

\end{tabular}}



\end{center}
\caption{\textbf{The results of all experiments with features.} In all experiment results with features, including the results of gpt-3.5-turbo-0613, llama-2-7b-chat, and llama-2-13b-chat. The table headers respectively represent three prompting strategies: Directly prompting, Oneshot prompting, and Chain-of-Thought prompting at three different similarity granularities: Large, Middle, and Small. The \textbf{bold number} indicating the best-performing model in the same strategy, and \underline{underline number} indicating the best-performing strategy in the same model.}
\label{tab:final_results}
\end{table}

==> tables/06_results/final_results_wo_features.tex <==
\begin{table}



\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{clccccccccc} 

\toprule
\multirow{2}{*}{\bf Category}          & \multirow{2}{*}{\bf Model} & \multicolumn{3}{c}{\bf Directly(w/o features)} & \multicolumn{3}{c}{\bf Oneshot(w/o features)} & \multicolumn{3}{c}{\bf CoT(w/o features)}  \\* 
\cmidrule{3-11}
                                   &                        & \bf Large     & \bf Middle     & \bf Small                      & \bf Large     & \bf Middle     & \bf Small                     & \bf Large     & \bf Middle     & \bf Small                  \\* 
\midrule
\multirow{4}{*}{\textit{Clothing}} & human                  & $93.51_{\pm 0.00}$ & $88.69_{\pm 0.00}$ & $66.53_{\pm 0.00}$                  & \textemdash & \textemdash & \textemdash                 & \textemdash & \textemdash & \textemdash             \\
                                    & gpt-3.5                & $\textbf{48.27}_{\pm 0.74}$ & $\textbf{50.83}_{\pm 0.56}$ & $\textbf{48.39}_{\pm 0.33}$                  & $45.74_{\pm 0.89}$ & $\underline{\textbf{54.45}}_{\pm 0.56}$ & $\underline{\textbf{50.07}}_{\pm 1.56}$                 & $\underline{\textbf{50.72}}_{\pm 0.41}$ & $\textbf{52.94}_{\pm 1.40}$ & $46.77_{\pm 1.06}$              \\*
                                   & llama-13b              & $46.10_{\pm 0.00}$ & $46.61_{\pm 0.00}$ & $46.37_{\pm 0.00}$                  & $\underline{\textbf{51.73}}_{\pm 0.00}$ & $\underline{51.13}_{\pm 0.00}$ & $49.80_{\pm 0.00}$                 & $48.26_{\pm 0.00}$ & $47.51_{\pm 0.00}$ & $\underline{\textbf{50.20}}_{\pm 0.00}$              \\* 
                                   & llama-7b               & $\underline{40.04}_{\pm 0.00}$ & $\underline{39.14}_{\pm 0.00}$ & $\underline{40.32}_{\pm 0.00}$                  & $26.62_{\pm 0.00}$ & $29.86_{\pm 0.00}$ & $31.65_{\pm 0.00}$                 & $37.45_{\pm 0.00}$ & $36.65_{\pm 0.00}$ & $39.72_{\pm 0.00}$              \\*
                                    
\midrule
\multirow{4}{*}{\textit{Food}}     & human                  & $91.67_{\pm 0.00}$ & $64.35_{\pm 0.00}$ & $67.55_{\pm 0.00}$                   & \textemdash & \textemdash & \textemdash                  & \textemdash & \textemdash & \textemdash              \\ 
                                    & gpt-3.5                & $\underline{\textbf{58.55}}_{\pm 0.30}$ & $\underline{\textbf{68.77}}_{\pm 0.00}$ & $\underline{\textbf{54.23}}_{\pm 0.37}$                  & $\textbf{51.39}_{\pm 0.60}$ & $53.04_{\pm 0.36}$ & $\textbf{49.90}_{\pm 0.37}$                 & $\textbf{49.36}_{\pm 0.91}$ & $50.72_{\pm 1.63}$ & $\textbf{51.87}_{\pm 0.87}$              \\*
                                   & llama-13b              & $\underline{48.08}_{\pm 0.00}$ & $50.22_{\pm 0.00}$ & $48.53_{\pm 0.00}$                  & $37.50_{\pm 0.00}$ & $\underline{\textbf{57.61}}_{\pm 0.00}$ & $\underline{48.67}_{\pm 0.00}$                 & $46.47_{\pm 0.00}$ & $\textbf{57.17}_{\pm 0.00}$ & $48.08_{\pm 0.00}$              \\
                                   & llama-7b               & $42.31_{\pm 0.00}$ & $40.65_{\pm 0.00}$ & $43.66_{\pm 0.00}$                  & $41.03_{\pm 0.00}$ & $31.96_{\pm 0.00}$ & $36.73_{\pm 0.00}$                 & $\underline{46.15}_{\pm 0.00}$ & $\underline{46.30}_{\pm 0.00}$ & $\underline{46.31}_{\pm 0.00}$              \\*
\bottomrule
\end{tabular}}



\end{center}
\caption{\textbf{The results of all experiments without features.} Based on the experiment in Table \ref{tab:final_results}, external features are removed from the prompt words.}
\label{tab:final_results_wo_features}
\end{table}

==> tables/06_results/geoculture_means_std.tex <==
\begin{table}[t]

\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccc} 
\toprule
\multirow{2}{*}{\bf Accuracy} & \multicolumn{3}{c}{\bf with features} & \multicolumn{3}{c}{\bf w/o features} \\
\cmidrule{2-7}
& \bf Eastern & \bf Western & \bf Across & \bf Eastern & \bf Western & \bf Across\\ 
\midrule
value & $53.84_{\pm 6.77}$ & $54.46_{\pm 8.11}$ & $54.52_{\pm 20.25}$ & $55.37_{\pm 8.65}$ & $52.46_{\pm 7.67}$ & $51.39_{\pm 18.96}$ \\
\bottomrule
\end{tabular}
}
    
\end{center}

\caption{\textbf{The accuracy of GPT when cultural concepts originate from within Eastern countries, within Western countries, and between Eastern and Western countries.} In different groups of experiments used to evaluate GPT, we notice that there are certain differences in the average accuracy between different geo-cultures. Moreover, when cultural concepts come from cultures between Estern and Western cultures, the standard variance reflects the model's differences between different cultures.}
\label{tab:geoculture_means_std}
\end{table}
